Machine Translation of Low-Resource Indo-European Languages

In this work, we investigate methods for the challenging task of translating between low-resource language pairs that exhibit some level of similarity. In particular, we consider the utility of transfer learning for translating between several Indo-European low-resource languages from the Germanic and Romance language families. In particular, we build two main classes of transfer-based systems to study how relatedness can benefit the translation performance. The primary system fine-tunes a model pre-trained on a related language pair and the contrastive system fine-tunes one pre-trained on an unrelated language pair. Our experiments show that although relatedness is not necessary for transfer learning to work, it does benefit model performance.

==> tables/baseline_comparison_contrastive.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%

==> tables/baseline_comparison_primary.tex <==
%
%
%
%
%
%
%
%

%
%
%
%
%
%
%
%
%
%

%
%
%
%

==> tables/contrastive_results_for_poster.tex <==
\begin{table*}
\centering
\begin{tabular}{Lc|cc|rrrrr}
\hline
\multicolumn{2}{c|}{\textbf{Non-language-related}} & \multicolumn{2}{c|}{\textbf{Before TL}} & \multicolumn{2}{c}{\textbf{After TL}} \\
\hline
\textbf{Pre-trained Model} & \textbf{Lang. Pairs} & \textbf{BLEU} & \textbf{chrF} & \textbf{BLEU} & \textbf{chrF}\\
\hline
ca-en & ca-it & 1.97 & 0.249 & \textbf{25.46} & \textbf{0.539}  \\
ca-en & ca-oc & 2.16 & 0.258 & \textbf{51.46} & \textbf{0.736}  \\
ca-en & ca-ro & 1.59 & 0.209 & \textbf{8.61} & \textbf{0.311} \\
\hline

\end{tabular}
\caption{Contrastive system reuslts for poster}
\label{tab:contrastive_reuslts}
\end{table*}

==> tables/primary_result_for_poster.tex <==
\begin{table*}[h]
\centering
\begin{tabular}{Lc|cc|rrrrr}
\hline
\multicolumn{2}{c|}{\textbf{Language-related}}&  \multicolumn{2}{c|}{\textbf{Before TL}} & \multicolumn{2}{c}{\textbf{After TL}} \\
\hline
\textbf{Pre-trained Model} & \textbf{Lang. Pairs} & \textbf{BLEU} & \textbf{chrF} & \textbf{BLEU} & \textbf{chrF} \\
\hline
ca-es & ca-it & 7.07 & 0.370 & \textbf{33.13} & \textbf{0.602}  \\
ca-es & ca-oc & 12.56 & 0.472 & \textbf{59.93} & \textbf{0.787}  \\
ca-es & ca-ro & 4.43 & 0.266 & \textbf{1124} & \textbf{0.354}  \\
\hline
\end{tabular}
\caption{Primary system results for poster}
\label{tab:primary_reuslts}
\end{table*}



%

==> tables/results_contrastive.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%

==> tables/results_primary.tex <==
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%
%

%
%
%
%
